New Definitions and Evaluations for Saliency Methods: Staying Intrinsic, Complete and Sound

Saliency methods compute heat maps that highlight portions of an input that were most {\em important} for the label assigned to it by a deep net. Evaluations of saliency methods convert this heat map into a new {\em masked input} by retaining the $k$ highest-ranked pixels of the original input and replacing the rest with \textquotedblleft uninformative\textquotedblright\ pixels, and checking if the net's output is mostly unchanged. This is usually seen as an {\em explanation} of the output, but the current paper highlights reasons why this inference of causality may be suspect. Inspired by logic concepts of {\em completeness \& soundness}, it observes that the above type of evaluation focuses on completeness of the explanation, but ignores soundness. New evaluation metrics are introduced to capture both notions, while staying in an {\em intrinsic} framework -- i.e., using the dataset and the net, but no separately trained nets, human evaluations, etc. A simple saliency method is described that matches or outperforms prior methods in the evaluations. Experiments also suggest new intrinsic justifications, based on soundness, for popular heuristic tricks such as TV regularization and upsampling.

==> mincircuit.tex <==
\section{Logic view of saliency methods: Partial assignments}
\label{sec:logic}
In general the saliency method is given a circuit $f$ (i.e., a deep net) and an input $x$, and  asked to identify a portion of $x$ "responsible" for the output of $f$ on $x$.
A running theme in saliency methods/evaluations is that the salient pixels should be sufficient to convince us about the model's output, regardless of contents of the other pixels. For instance, greying out the pixels (or setting them to average pixel value) that are identified as non-salient should have very little effect on the output. This idea appears in many saliency methods (and evaluation metrics), including Shapley values and mask-based explanations. (NB: detractors point out that typically the circuit was not trained using such partial assignments. But in practice trained circuits gives meaningful outputs on partial assignments.)  Now we mathematically formalize this.

\begin{definition}(Partial assignments) \label{def:partialassign} A {\em partial assignment} $(\pi, S)$ {\em consistent with input $x$} consists of a subset $S$ of pixel locations and an assignment $\pi$ of values to pixels that agrees with $x$ on pixel locations in $S$ and assigns the default value to every pixel in $\overline{S}$.  The {\em size} of the partial assignment is $\abssm{S}$. If $\pi$  causes $f$ to output $a$ then it is said to {\em validate} the value $a$ {\em for} $f$ on $x$. 

\end{definition}
Thus a (simplified) view of many saliency methods is that given $f, x$ and a target value $a$ they try to generate a partial assignment consistent with $x$ that validates $a$. The next definition adapts completeness/soundness terminology from logic to articulate an intrinsic notion of correctness for such a method. Note that the trivial method that declares all input coordinates as salient is complete and sound. Ideally saliency methods should be complete and sound using a smaller partial assignment.

\begin{definition}(Completeness/Soundness) \label{defn:logiccomplete}
 A saliency method is given $f, x$ and a label $a$.
 %and produces a partial assignment consistent with $x$. 
 %{\em complete for a class of $\mX$ of inputs and class $\mF$ of circuits} if for every $f \in \mF, x \in \mX$ it finds a partial assignment consistent with $x$ that validates the value $f(x)$.  %\in \mX$. 
 The method is {\em complete on $f, x$} if it finds a partial assignment consistent with $x$ that validates the value $f(x)$. 
 The method is {\em sound on $f, x$} if it cannot find a partial assignment to validate a value $a$ different from $f(x)$. 
 %(An alternative definition allowing occasional errors: for every $f \in \mF$ allow failure for a negligible fraction of  $x$'s.)
% Completeness and soundness are analogously defined for evaluations of saliency methods.
\end{definition}
\noindent{\em Notes:} (i) Many intrinsic saliency methods yield a heat map, which can be viewed as a  partial assignment with fractions (indicating "importance") associated with coordinates of $S$. But the heatmap may not yield a satisfying assignment to the circuit. (ii) Heatmaps are problematic in an intrinsic (as opposed to human-oriented) framework because  in highly nonlinear model,  the "meaning" of fraction $0.4$ in a coordinate has different meanings depending upon the
weightings to {\em other} coordinate. The statistical framework of Section~\ref{sec:stat} will  integrate heatmaps as well. %\ns{heatmap can be converted to a randomized partial assignment. implicit in some AUC metrics. most intrinsic metrics involve some discretization step anyway, so this partial assignment framework is relevant}
%(iii) The trivial saliency method that reports all pixels to be salient satisfies completeness and soundness. 
(iii) In several existing backpropagation-like saliency methods, completeness is not assured  and the term is used in those papers to refer to a very different property: sum of saliency scores adds up to the logit associated with the label.  This property ensures "Soundness" in our sense. (iv) Conversely in mask-based saliency methods, completeness is often assured almost by definition of procedure,  and ensuring soundness takes some care (see Figure~\ref{fig:ghostandreal}) as we will later see. 
%\ns{(vi) out-of-distribution issue with trained models.}
%for why soundness is  
%\ns{Trivial way to ensure soundness. Thus any method}
%and this information (together with the information that pixels in $\overline{S}$ receive a default value) is enough to fix the output of the circuit to the desired value. 

\begin{figure}
	\centering
	\includegraphics[scale = 0.40]{ghostandreal2.pdf}
		\caption{Methods to find partial assignments may not be sound. (i) CIFAR10 image (ii) partial assignment consistent with it, validates label "dog" (iii) partial assignment that validates label "horse."}
		\label{fig:ghostandreal}
	\end{figure}


\iffalse Saliency typically highlights a portion of $x$ that ``explains'' the final label.
 and grey/gaussian values in the rest is like a {\em minimal} satisfying assignment to the circuit.the pixel assignment consisting of $\pi$ in the salient pixels and grey/gaussian values in the rest is like a {\em minimal} satisfying assignment to the circuit. \fi 

%Implicitly, research in saliency methods has been viewing the salient portions identified in the input as a {\em sufficient justification} for the label output by the net. 
 
 
  Thus the crux is designing sound and complete methods that find short partial assignments.  The next result shows this is computationally very difficult in general.
  Similar ideas also show the difficulty of a problem used in the popular {\em deletion} metrics used in saliency evaluation.
  %\ns{minimality is encouraged in all masking methods through $\ell_1$
 %regularization}  %(The theorem assumes 
  %computcan be very difficult. 
  %It concerns the computational problem where  saliency method is given a ReLU circuit implementing $f\colon \{0,1\}^n \to \{0,1\}$ and an input $x$.  The default value for input coordinates is $0$. 
 
 %{\sc note that backprop like methods probably satisfy soundness by definition. And "completeness" means something else there!}
% The above definition required completeness and soundness only for certain classes of circuits and inputs (e.g., circuits produced by usual deep learning). The next theorem says that if we allowed all circuits this makes the problem intractable.
 
 \begin{theorem}(See Appendix \ref{sec:NPHardTheorem}) \label{thm:intractability}
 The following two problems are NP-hard on ReLU circuits for every constant $C_1, C_2>1$: To find  (i) a validating partial assignment $(\pi, S)$   of size at most $C_1\cdot K_1$, where $K_1$ is the size of the smallest partial assignment that validates the value $f(x)$. (ii) a set $S_2$ of size $C_2 K_2$ such that assigning grey values in $S_2$ makes the circuit evaluate to a different value than $f(x)$, where $K_2$ is the minimum size of such a set. 
 %(Here default value is $0$.) 
 \end{theorem}

Of course, NP-hardness result  only concern worst-case complexity and presumably  deep learning on natural images is not a worst-case scenario. The takeaway from  Theorem~\ref{thm:intractability} is that usual saliency methods (which do run in time polynomial or even linear in the size of the circuit) are not guaranteed to find anything remotely resembling the shortest  partial assignments  without making additional assumptions about the circuit or the class of inputs. While basing saliency methods on axiomatic characterizations 
%"contribution" of an that 
can instill some rigor, this will not imply  even approximate minimality for the  saliency maps they lead to. Part (ii) similar cautions about the difficulty of the deletion metric.

% for general ReLU circuits.

Appendix \ref{sec:backpropsalmincert} gives simple examples on which backpropagation-style saliency methods can fail to find minimal certificates or anything close to them. 



==> old-mona-lisa-phenomenon.tex <==
\section{Mona Lisa smile phenomenon}
	{\sc this section shows existence of short sufficient certificates, in a statistical sense.}
	
	Imagine that $\DataX$ is the set of real images of cats and dogs. We see every image $\vx \in \DataX$ as a vector in $\R^d$ and we use $x_i$ to denote the value of the $i$-th pixel of $\vx$. The ground truth for an image $\vx$ is denoted by $g(\vx) \in \{\pm 1\}$, where $1$ stands for the cat and $-1$ stands for the dog.
	
	Together with the ground truth $g(\vx)$, we also assume that there is a ground truth explanation: for each image $\vx$ the explanation consists of a subset of pixels and the assignment of values to them in $\vx$, and it is sufficient for a human to consider $\vx$ as an image in the class $g(\vx)$ if he/she only sees the subset of pixels $S$ in $\vx$.
	Formally the explanation for an image $\vx$ is a tuple $\pi^*(\vx) := (S(\vx), \vx[S(\vx)])$, where $S(\vx) \subseteq [d]$ and we use $\vx[A]$ to denote the matrix whose entry at $(i, j)$ is $x(i,j)$ if $(i, j) \in A$ and $0$ otherwise. One could in principle estimate this explanation using human studies.
	
	\kaifeng{$0$ here can be replaced by any other number. Maybe $-1$ or $\infty$ is better because they are out of the range of valid pixel values.}
	
	In traditional logic, where inputs are bit strings and the classifier is a boolean function these would be min-terms, and the function can be written as OR of these.
	
	\begin{assumption} \label{ass:overlap}
		For almost all $\vx$, $\vx'$ that have different labels, their explanations have small overlap. That is, for all $\vx, \vx' \in \DataX$, if $g(\vx) \ne g(\vx')$, then \[
			\frac{\sum_{i \in S(\vx) \cap S(\vx')} \onec{x_i \ne x'_i}}{\min\{\abs{S(\vx)}, \abs{S(\vx')}\}} < p,
		\]
		where $p \in [0, 1)$ is some threshold value depending on the task.
	\end{assumption}

	\kaifeng{I replaced ``For almost all $\vx_1$, $\vx_2$'' by ``For all $\vx_1$, $\vx_2$'' for simplicity.}
	
	\begin{theorem}
		Under \Cref{ass:overlap}, for any set of images $\DataT \subseteq \DataX$, we can choose $\hat{S}(\vx) \subseteq S(\vx)$ for each $\vx \in \DataT$, such that $\abssm{\hat{S}(\vx)} \le O(\log\abssm{\DataT})$ and for all $\vx, \vx' \in \DataT$, if $g(\vx) \ne g(\vx')$, then $\vx[\hat{S}(\vx)] \ne \vx'[\hat{S}(\vx)]$.
	\end{theorem}
	\begin{proof}
		We can prove via probabilistic method. For every $\vx$,
		\begin{itemize}
			\item Initilize $\hat{S}(\vx) \gets \varnothing$;
			\item Repeat the following for $K := \left\lceil\frac{\log \abssm{\DataT}}{\log(1/(1-p))}\right\rceil$ times:
			\begin{itemize}
				\item Randomly select an element in $S(\vx)$;
				\item Add the selected element to $\hat{S}(\vx)$ if it is not present.
			\end{itemize}
		\end{itemize}
		For every $\vx' \in \DataT$ with a different label, by \Cref{ass:overlap}, the probability of having $\vx[\hat{S}(\vx)] = \vx'[\hat{S}(\vx)]$ is no greater than $(1-p)^{K} < \frac{1}{\abssm{\DataT}}$. Taking the union bound, we know that
		\[
			\Pr\left[\exists \vx' \in \DataT: g(\vx) \ne g(\vx'), \vx[\hat{S}(\vx)] \ne \vx'[\hat{S}(\vx)]\right] < \frac{1}{\abssm{\DataT}} \cdot \abssm{\DataT} = 1.
		\]
		This means this algorithm can construct $\hat{S}(\vx)$ that matches with the claim of the theorem with non-zero probability. So we can construct $\hat{S}(\vx)$ by running this algorithm repeatedly until it succeeds.
	\end{proof}
	
	In particular, note that by VC theory it suffices to let T be O(net size × \# pixels).
	
	Consequence 1: Usual saliency methods don’t need to return human interpretable
	explanations.
	(Can back this up with an analysis of logistic regression or least squares regression.)
	
	Consequence 2: Saliency methods also have the same limitation a priori. In other words the axiomatic approach grounded in cooperative game theory does not guarantee human- interpretable explanations.
	Proposed method to find human-interpretable explanations: Train as usual and find saliency maps. Take a class and gray out most salient pixels. For other classes gray out random pixels (or contiguous perhaps). Train a classifier to recognize the class, and find its salient pixels. Do this for a few rounds.The final map is some kind of avg of saliency maps from the rounds.

==> oldintro.tex <==
\section{Introduction}
\label{sec:intro}
{\em Why did the deep net give a certain answer on a particular input, and can we trust the answer?} {\em Saliency methods} try to provide explanations, and are thus of great interest from viewpoint of human explainability, fairness,  robustness, etc.
 %tend to fall They broad definitions in machine learning. The first is visual human saliency, which attempts to predict which portions of an input, e.g. objects in a video, most capture human attention. We deal instead with the second definition, which is broadly, given 
This  paper restricts attention to methods that 
%an input, e.g. an image, and a model, 
return an importance score for each coordinate of the input ---usually visualized as a  heat map--- that captures its importance to the final decision.\footnote{Heat maps suffice for recognition/classification tasks; other tasks may require more complex explanations.} %Often the sum of the scores equals the final decision (decision could be the output probability, or  corresponding logit).
We refer the reader to \citet{samek2019explainable} for an extensive survey and Section~\ref{sec:prior} for a short account of such methods and controversies.


There are two important components in the research on saliency: {\em saliency methods} that produce such heat maps for explanations, and {\em saliency evaluation metrics} that aim to test and compare  saliency methods.
Numerous saliency methods have been proposed to learn such heat maps. 
Some methods learn maps through ``credit attribution'' to individual input coordinates by using methods reminiscent of backpropagation \citep{binder2016layer,selvaraju2016grad}, while some are derived using careful axiomatization of credit assignment using the idea of Shapley values from cooperative game theory \citep{lundberg2017unified,yeh2020completeness}.
Some recent methods  train another deep net to produce  heat maps \citep{dabkowski2017real,phang2020investigating}.
Given the proliferation of saliency methods, an ecosystem of evaluation metrics has emerged to  evaluate the quality of explanations produced by saliency methods, either through human evaluations \citep{adebayo2018sanity}, comparison to certain ground truth explanations \citep{zhang2018top} or other evaluations that do not require any external annotation or supervision \citep{dabkowski2017real} \citet{petsiuk2018rise}.


%\vspace*{-0.1in}
%\subsection*{This paper}
%\vspace*{-0.1in}
In this paper we restrict attention to a class of evaluations we refer to as
{\em intrinsic}, that aim to evaluate saliency maps based on whether they are good explanations for the model prediction.
These only involve computations using the provided heat map and the net, and do not involve extrinsic factors such as human judgements or retraining.  A popular idea in such evaluations (see \Cref{sec:stat} for references) is to create a new composite input ---or sequence of such inputs--- using the heat map and the original input, and to evaluate the original net on this composite input. For example, if $M$ is a binary vector with $1$'s in the $k$ coordinates with the highest values in the heat map, then $x \odot M$ (with $\odot$ denoting coordinate-wise multiplication) can be viewed as a composite input\footnote{When $x$ is an image the zeroes in this masked input are often replaced with gray values.} (aka ``masked input'') that can be fed into the original net. By varying $k$ one obtains a sequence of masks $M$.
Although there is an issue of distribution shift due to the net never having trained on composite inputs, in practice, especially for image data, trained nets work fine on masked inputs. (This is also exploited in Shapley value based saliency methods.) 

Inspired by logical reasoning, we identity a key component missing in existing {\em intrinsic evaluations}: {\em soundness} of the saliency method.
In simple terms, checking soundness for mask-based explanations entails verifying that it is impossible for the method to produce well-performing (in the composite-input evaluations) heat maps corresponding to the {\em incorrect}
%\dy{we should change a name for this, maybe \emph{unfavored} or \emph{unpopular}?}
labels, i.e. labels not predicted as the most likely by the model.
By contrast current masking evaluations focus on a property akin to {\em completeness}\footnote{In the literature devoted to saliency methods based upon backpropagation-like procedure, such as {\sc Gradient $\odot$ Input} or LRP, the term {\em completeness} is used in a slightly different sense: the sum of the heat map values has to be equal to the logit value for the label.} in logic: the heat map ``justifies'' the correct label, i.e. the label judged to be most likely by the model. 
%\revise{In logic, {\em completeness} of a proof system roughly means that ``you can prove any true statement'' and {\em soundness} means that ``you cannot prove any false statement''.
%Analogously for saliency if a model that predicts label $a$ for input $x$, we want the saliency method to be able to produce an explanation for the true statement that ``model predicts label $a$ for input $x$'' (completeness), but should be unable to produce an explanation for a false statement ``model predicts label $a'$ for input $x$'' where $a'\neq a$ (soundness).}
We argue that soundness can be a useful criterion in addition to completeness.

\revise{The concept of soundness is motivated by observing that the recent mask-based saliency methods are inherently different from the earlier gradient-based methods.
They produce a heatmap that is interpreted as a masked image that, when fed into the net must make it output the same label that received the top logit value on the full image.
Our paper observes that it is unclear at a logical level why this should be considered an ``explanation'', since to be convinced one must verify that a different mask could not induce the net to output a label corresponding to other logits.
\Cref{fig:artifact-small} shows that in fact this issue is real; masks do exist that can ``justify'' the wrong labels.
We introduce soundness as a quantitative measure for this issue (definitions in \Cref{sec:completeness_and_soundness}), and propose that evaluations of mask-based saliency methods should account for soundness.}
%Soundness can be viewed as a reassurance that there is no way to cheat the evaluation in case of an incorrect label.
Many past works allude to difficulty of the soundness concept, mentioning that computations to find the ``best" mask end up finding artifacts that can even justify labels that are obviously incorrect.
To avoid uncovering artifacts, the methods to find masks/heat maps use a suitable regularization (usually TV).
However, \Cref{fig:artifact-small} illustrates that TV regularization is not a full solution to removing artifacts. 



Another reason for incorporating soundness with completeness in metrics is to implicitly encourage saliency methods to also produce saliency maps for incorrect labels.
When using the classifier in the wild---as opposed to on a dataset with centered images--- we might encounter multiple salient objects in the image, and the net may not have high confidence in a single label.
It would then be reasonable to have saliency methods find evidence for all the labels which the net outputs with reasonable confidence.
\revise{We find in \Cref{fig:elezeb} that our saliency method that produces masks for all labels can produce different and meaningful masks for different labels when there are multiple objects present in the image\footnote{\revise{In this paper, multiple objects in one image is not formally considered, as we assume single object classification is the prior knowledge. Therefore, either zebra or elephant in \Cref{fig:elezeb} is regarded as an incorrect label. A quick extension to the multi-object case is to define correct labels as the labels whose model probability exceeds a certain threshold. 
%Then the new definition will expect a good saliency method to provide masking explanations for elephant and zebra respectively as long as the model probability for elephant and zebra are high enough.
Even without the extended definition of correct labels, \Cref{def:soundcompletestat} with suitable $\alpha, \beta$ already allows explanations to exist for both elephant and zebra as long as the model probability for elephant and zebra are high enough.} }, compared to prior state-of-the-art methods, that output a single mask for all labels that contains both objects (more on this in \Cref{sec:elezeb}).}


%The soundness requirement is important for a variety of reasons. First, when using the classifier in the wild---as opposed to on a dataset with images of centered main objects--- we will encounter multiple salient objects in the image, and the net may not have high confidence in a single label. Then it would be reasonable to have saliency methods find evidence for all the labels present in the image.
%\revise{In fact, we find in \Cref{fig:elezeb} that our method (from \Cref{sec:procedures}) that produces masks for all labels can produce different and meaningful masks for different labels when there are multiple objects present in the image, compared to prior state-of-the-art methods, that output a single mask for all labels that contains both objects.}
%%Clearly, the goal of the saliency evaluation is to exhibit that the portion of the input found to be most important by the saliency method (i.e., $M$) was actually sufficient --- or necessary, in some evaluations --- for deciding on the label that was originally output by the net.
%\revise{Moreover, }
%%But
%a more subtle reason for soundness is
%%that appears to have gone unaddressed in past discussions is 
%why human overseers ---who figure nowhere in an intrinsic evaluation--- should consider the heat map as a demonstration of correctness of the classification. %Inspired by logical reasoning, one can identify both a {\em completeness} and a {\em soundness} aspect to correctness. We give an intuitive introduction, leaving formal definitions to Section~\ref{sec:completeness_and_soundness}.
%%{\em Completeness} would require that if the net's answer is correct, it should be possible for the saliency method to identify a mask $M$ (or a sequence of such masks) such that the masked input also gets the same label.  Current evaluations satisfy completeness in this sense. 
%%{\em Soundness} would require that the evaluation method would be able to reject any presented mask for any label that was not output by the net.  This is usually not checked in current evaluations. 




\iffalse
The soundness issue in practice is illustrated in \Cref{fig:artifact-small} using CIFAR-10 images.  For both images, a simple saliency method (\Cref{sec:procedures}) can be used to construct masked inputs that can cause the classifier net to output the incorrect label (w.r.t. model prediction) with significant probability, in addition to constructing a good mask for the correct label.
The soundness condition we suggest requires that the acceptance probability on composite input should not grossly outstrip the acceptance probability on the unmasked input; see Section~\ref{sec:completeness_and_soundness} for precise definitions.
\fi

%with the highest probability.
%\Cref{fig:artifact-small} the label output by the net was correctly computed by the classifier net and the mask output by the saliency method does indeed  this.
% ; we elaborate on this in \Cref{sec:soundness_completeness}.
%This notion of soundness inspires both, a new metric of evaluation of saliency maps and also a method for computing saliency maps.
%We delve deeper into the concept of soundness before detailing our main contributions.
% At first sight such an evaluation might not make sense since the net was never trained on such composite inputs. However, in practice, especially for image data, the trained nets work fine on masked images.
% Similar composite inputs are also used in saliency methods based upon Shapley values \ns{cite}.

%{\sc removed para about controversies that can move into a later section}
\iffalse 

\ns{this next paragraph seems somewhat orthogonal to the current story, perhaps not required here?.}
\myparagraph{Difficulties in defining/evaluating saliency: a taste.}
We give an example to illustrate the difficulties in this field. %which methods need to. %end up having to do. 
Suppose the net's input consists of bit strings,  and it outputs $1$ iff at least $4$ input bits are $1$. (This is a toy example of a concept that can be recognized if at least $4$ out of $9$ features are present.) What should be the saliency map for an input in which $9$ bits are $1$? Logically speaking,  highlighting any $4$ bits that are $1$ is enough to justify the answer of $1$. {\em Shapley values} would give equal saliency to all $9$ bits that are $1$. (For simplicity we ignore  complicated Shapley variants.) 

%A large subclass of intrinsic methods are backpropagation-like and do credit attribution roughly inspired by gradient of output with respect to input. %$\partial \text{output}/\partial \text{input}$, 
Backpropagation-like methods can give a variety of answers depending upon their details (See \Cref{sec:backpropsalmincert} \kf{need to reword there because this section does not support this directly}), and the final saliency map often depends upon how the net implemented its functionality (as opposed to just the input-output behavior). Various evaluations also have disparate expectations of when a map is good. For instance ROAR evaluation~\citep{hooker2019benchmark}, which is intrinsic, would reject maps containing fewer than six $1$'s, because it zeroes out (or greys out in case of image data) coordinates identified as most salient,  and checking if the answer on the modified input became $0$.
\fi 
\begin{figure}[t!]
\begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{ghost_small.png}
\end{subfigure}

\begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{ghost_small_bird_frog.png}
\end{subfigure}
    \caption{Masked CIFAR-10 images generated by our procedure with $\lambda_{TV} = 0.01$ shows the artifacts exist for masks generated for incorrect labels. More examples can be find in \Cref{fig:artifact} in Appendix. The base classifier outputs the correct label on the original image (ship and bird resp.) with probability at least 0.99, and assigns probability at most $10^{-5}$ for the incorrect label (cat and frog resp.). With the generated masks, the AUC metric for the correct label remains high (around 0.94 and 0.90), which corresponds to {\em completeness}, but AUC metric for the incorrect label rises tremendously (around 0.18 for cat mask, 0.71 for frog mask.) This suggests violation of {\em soundness}. }
    \label{fig:artifact-small}
    \vspace{-0.2in}
\end{figure}

%\myparagraph{Soundness and completeness of a saliency evaluation:}
%\label{sec:soundness_completeness}

%As mentioned earlier, this paper focuses on evaluations that feed a composite input/image $x \odot M$ to the original net, where $M$ is a binary vector produced by the saliency method being evaluated.





%There could be other reasons to require some form of soundness condition in saliency evaluations. For instance, while using the classifier in the wild ---as opposed on a dataset with images of centered main objects--- multiple objects may be present in the image, and the net may not have high confidence in a single label. Then it would be reasonable for saliency methods to find evidence for all the labels present in the image. 



\iffalse
\ns{
we can take any method and make it sound

language: $(x,f(x))$, prover: saliency method, verifier: any standard metric like AUC, proof: for any $(x, a)$ it is the mask $M(x, a)$

$M$ is an algorithm that runs on $(x, a)$.

our goal here is to evaluate a prover (or prover family)

completeness: whenever $a = f(x)$, the verifier (AUC score) should get high probability when the proof $M(x,a)$ is used.

soundness: whenever $a \neq f(x)$, then what??

ideally the prover should try to give the best proof for any $(x, a)$ that it can, and that shouldn't be good enough to prove when $a \neq f(x)$.
suppose the best algorithm was used to find the proof $M(x,a)$, then completeness and soundness are actually evaluating a metric rather than method.
checking if a metric is sensitive enough to be able to match the networks predictions. but again there is a cheating method which is to output $f(x)$ itself. so why are masks relevant?
}
\fi
  
  
  

\begin{figure}[htbp] 
	\centering
	\vspace{-0.2in}
	\includegraphics[width=0.5\textwidth]{elephant-zebra.png}
	\caption{Images containing both elephant(s) and zebra(s), and the corresponding masked ones generated by our method and the best-performing CA model in \citet{phang2020investigating}. The masks by \citet{phang2020investigating} are identical for different labels, and contains both elephant and zebra. In contrast, our method outputs descent masks for elephant and zebra accordingly.  }
	\vspace{-0.1in}
	\label{fig:elezeb}
\end{figure}
  
  
	\vspace{-0.1in}
\myparagraph{Main contributions:}
%Motivated by the distinction between completeness and soundness, the paper makes following other contributions.
\revise{
In this paper we make a case for pushing saliency methods and metrics to incorporate soundness in addition to completeness.
We propose metrics and a method and experimentally evaluate them in comparison to previous methods and metrics, leading to some novel findings.
Our main contributions are as follows:
}

	\vspace{-0.1in}
%Motivated by the above discussion, here are our contributions
\begin{itemize}[leftmargin=*]

    \item A new single number metric named {\em \cs{}} that evaluates the completeness and soundness simultaneously. It measures the probability that the saliency map for the model prediction has the best quality compared to all other labels. See \Cref{sec:consistency-score} for a formal definition.

    \item A saliency method in \Cref{sec:procedures} that bears similarity to prior works that learns masks through optimization, but with subtle differences.
    One of the differences is based on the logic of soundness: we learn a mask by trying to maximize the probability for the given label, rather than matching the probability, and learn the {\em best mask} for all labels this way.
    \revise{We find in experiments (\Cref{sec:expers}) that our method not only performs comparably to prior masked-based methods on earlier saliency metrics, but also does better than those methods on the proposed consistency score.}
    %Another difference is that we use random images to fill in pixels not in the salient set when computing the objective.
    %In \Cref{tab:imagenette_main}, our method shows better soundness than previous methods, while decently matching performance existing metrics.

    \item Previous works proposed ``tricks'' like TV penalty and upscaling of masks \citep{fong2017interpretable,dabkowski2017real} that are motivated by their ability to avoid ``artifacts'' and make the saliency maps visually look better.
    These justifications, however, are not in the spirit of an intrinsic evaluation of saliency maps.
    In this paper, we provide a novel {\em intrinsic} justification for these choices of TV penalty and upscaling, by showing that they improve the saliency maps by making them more sound, as empirically demonstrated in \Cref{sec:expers}.
    We complement this finding with a theoretical result in \Cref{sec:linear} that proves that TV regularization can help with soundness in a simple linear classification setting.
\end{itemize}

	\vspace{-0.1in}
\myparagraph{Paper outline:} \Cref{sec:prior} discusses prior works on saliency methods and evaluations. \Cref{sec:stat} delves further into the concept of completeness and soundness in the context of saliency evaluation, and describes our proposed metric of \cs{}. \Cref{sec:procedures} describes our saliency method and how it differs from prior approaches. Finally \Cref{sec:linear} describes various supportive experiments.


	\vspace{-0.1in}





%\section{Old Introduction}
% \kf{Old Intro Commented out.}

\begin{comment}
{\em Why did the deep net give a certain answer on a particular input?} {\em Saliency methods} try to provide explanations, and are thus of great interest from viewpoint of human explainability, fairness,  robustness, etc..\
 %tend to fall They broad definitions in machine learning. The first is visual human saliency, which attempts to predict which portions of an input, e.g. objects in a video, most capture human attention. We deal instead with the second definition, which is broadly, given 
This  paper restricts attention to methods that 
%an input, e.g. an image, and a model, 
return an importance score for each coordinate of the input ---usually visualized as a  heat map--- that captures its importance to the final decision.\footnote{Heatmaps suffice for usual recognition/classification tasks, but other ML tasks might require more complex explanations.} %Often the sum of the scores equals the final decision (decision could be the output probability, or  corresponding logit).
See \citet{samek2019explainable} for an extensive survey %of saliency methods and 
and Section~\ref{sec:prior} for a short account of methods and controversies. It will be good to differentiate between {\em saliency methods} ---which produce the heat map--and the {\em evaluations} of such methods. 


%We identify  two conceptually different classes of saliency methods, though their aims and methodologies (especially evaluation methodologies) of course overlap. 

%they explain the basis of an ML model's decision  by diving inside the model's computation to tease out the coordinates in the input that were most ``salient'' to the output. 

%, especially around the issue of how to evaluate saliency methods. 

The first class can be thought of as {\em intrinsic methods}: they explain the basis of an ML model's decision  by diving inside the model's computation to tease out the coordinates in the input that were most ``salient'' to the output. Doing so relies upon some {\em a priori} mathematical definition of each coordinate's ``contribution'' to the final output. Many intrinsic methods are reminiscent of backpropagation  and do "credit contribution" to each coordinate of the input roughly guided by gradient of the output with respect to the input. Some  intrinsic methods (a notable example being those relying on Shapley values from cooperative game theory) are derived from a careful axiomatization of credit attribution.
%the latter deal with the fact that the internal computation in a complicated model (say, deep net)   may not map well to human reasoning.


We refer to the second class of saliency methods as {\em human-oriented}: they avoid an {\em a priori} notion of ``contribution'' of individual coordinates of the input, and focus on 
producing human-interpretable {\em localization} of the portion  of the input germane to the output label. Recent successful methods (descended from a long tradition in computer vision) even end up  training another deep net (!) to use the classifier to compute a human-interpretable heat-map of the image regions that explain the output. Such methods do very well on a host of evaluation benchmarks, including their ability to mimic human-generated explanations. 
%There are many definitions of what should be considered important, and corresponding saliency methods have been constructed.
	
The current paper's ideas belong philosophically in the intrinsic tradition:  saliency of coordinates is defined via mathematical/logical notions that only reference the trained model. 

\iffalse
But the underlying concept of a partial assignment is very close to the masking-based concepts popular in human-oriented methods and shares their utility. We hope our formalization ---as well as supporting experiments and theory highlighting its properties--- begins to bridge the two classes of work. 
\fi

\myparagraph{Ground truth versus maximal labels versus target label.}
We evaluate both on images which the model classifies correctly, and those that it missclassifies.  Many saliency methods assume the ground truth label may not be available at test time, and we follow suit.


\myparagraph{Defining Instrinsic Saliency.}
The goal of extrinsic saliency is to highlight some relevant portion of the original input image. Given an orignal image, $X$ and a mask $M$, one can construct an image with super-imposed mask $X \odot M$ that a user may use to understand why the model made a particular decision. 
Intrinsic saliency, on the other hand, disregards use to the user, and instead has the goal of explaining a model's decision. Hence, if a model is confident on some logit $s_y$, i.e. $s_y$ is reasonably large, the saliency method should return a map certifying the value  $s_y$ (i.e. such that $f(X \odot M)$ is reasonably large). On the other hand, if $s_{y'}$ is small for some other logit, then the saliency method should not be able to find a mask $M'$ such that $f(X \odot M')$ is larger than $s_{y'}$.  If it does, then the saliency method may be explaining a belief that the model doesn't have, which would make us suspicious of its explanations in general. 

\myparagraph{Evidence of artifacts.}
Several previous works have noted the effect of mask artifacts. \citet{fong2017interpretable} noted that in an image of a maypole, the imposed mask may draw an irregular shape in the sky. \citet{dabkowski2017real} note that masks may have 'adversarial' artifacts, consisting of a few pixels that go unnoticed to humans but could destroy the model prediction. \\
Our understanding of artifacts, different from previous approaches, extends to the wrong label. Specifically, we find that un-regularized masks can be so powerful as to construct a phantom certificate for the wrong label (where $s_{y'}$ is small) such that $X \odot M'$ is large, and the resulting mask is non-trivial (consists of more than a few pixels, and can even resemble another image class.) 




Motivated by the previous observation, we consider saliency methods that learn a mask (and hence do not automatically satisfy completeness.) We introduce the notion of \emph{soundness}, that a masking method should not be able to construct a convincing explanation for the wrong label. 

We use this notion both to evaluate existing saliency methods, and to explain intrinsically various heuristic tricks that previously had only extrinsic explanations. 
%and   {\em human-oriented methods}, especially popular in computer vision, NLP etc., which try to generate human-interpretable maps and are often even evaluated with respect to ability to mimic human explanations. The two classes can and do overlap.
%Most intrinsic methods 

\myparagraph{Difficulties in working on intrinsic methods.}
A simple example can illustrate the difficulties in defining saliency  from first principles, which intrinsic methods need to. %end up having to do. 
Suppose the net's input consists of bit strings,  and it outputs $1$ iff at least $4$ input bits are $1$. What should be the saliency map for an input in which $9$ bits are $1$? Logically speaking,  highlighting any $4$ bits that are $1$ is enough to justify the answer of $1$. {\em Shapley values}, a concept from cooperative game theory, would give equal saliency to all $9$ bits that are $1$. (For simplicity we ignore here more complicated Shapley variants.) 
%A large subclass of intrinsic methods are backpropagation-like and do credit attribution roughly inspired by gradient of output with respect to input. %$\partial \text{output}/\partial \text{input}$, 
Backpropagation-like methods can give a variety of answers depending upon their details (See \Cref{sec:backpropsalmincert}), and  the final saliency map often depends upon how the net implemented its functionality (as opposed to just the input-output behavior).  The ROAR evaluation~\citet{hooker2019benchmark} would reject  maps containing fewer than six $1$'s, because it zeroes out (or greys out in case of image data) coordinates identified as most salient,  and checking if the answer on the modified input became $0$. 

%{\sc (Aside: Can we check if there are some backprop like methods that give absolutely the wrong answer, e.g. saliency to a coordinate that is $0$?)} 

%For tasks in computer vision and NLP a key objective for the saliency map is to  convince  humans that an ML model computed correctly.   This runs into the issue that a deep net's internal computation may not map well to human reasoning, and so recent successful methods \cite{} (descended from a longer tradition in computer vision) end up having to train another deep net (!) to use the first deep net to compute a human-interpretable heat-map of the image regions that explain the output. These methods do well on a host of evaluation benchmarks. 






\iffalse 

Main idea is that implicitly designers of saliency methods have been thinking of the salient portions identified in the input as a sufficient justification for the label output by the net. In other words, if $x$ is the input, and $\pi$ gives the locations and values of its most salient pixels then the pixel assignment consisting of $\pi$ in the salient pixels and grey/gaussian values in the rest is like a {\em minimal} satisfying assignment to the circuit. 
\fi 


\myparagraph{Why we focus on masking methods.}
We define masking methods similarly to \citet{phang2020investigating}; a method that attempts to learn a mask $M$ given a model $f$ and input(s) $X$. Some simple methods like LRP and Gradient $\odot$ Input for ReLU networks with no bias satisfy completeness and soundness already. However, masking methods are considered state of the art, and our focus in this work is assessing the extent to which these satisfy soundness. 

\myparagraph{Our Contributions.}
a) We introduce and motivate soundness. Since a mask-based saliency map can be viewed as a portion of the input that "certifies" the correctness of the net's output, we can view this certificate as part of a probabilistic proof system. This motivates notion of completeness (which has been discussed in previous works) and our new contribution of soundness for the saliency map. 
b) Provide a new metric (i.e., a single number) for mask-based saliency methods, which can be used to compare methods. Evaluating this metric gives new insights into efficacies of current saliency methods. 
c) We advocate for methods and evaluations for mask-based saliency  that are intrinsic ---use just the training dataset and the trained net, and does not use separately trained nets, distractor distributions, human evaluations etc. To this end, we introduce a new saliency method that does not require additional training of infillers and is fairly simple as well. 
\iffalse
We view the classifier as a circuit acting on the input.  %extends this notion to the statistical setting more relevant to machine learning. 
A central idea is a notion of saliency that involves  partial assignments that validate the label output by the circuit. This is an intrinsic notion, but  very analogous to popular {\em mask-based} explanations in the human-oriented category. (a) Sections~\ref{sec:logic} views partial assignments as precise logical concepts and defines {\em completeness} and {\em soundness} for procedures that find them. Existing saliency methods focus on at most one of these two notions, whereas both are needed.  Section~\ref{sec:stat} extends the framework to statistical learning and relates completeness and soundness to existing evaluation metrics. (b) Section~\ref{sec:logic} shows that even finding weak approximations to short partial assignments (or to deletion metrics) is computationally intractable (i.e., NP-hard) for general circuits. %of the existing saliency methods (which run in time polynomial or even linear in the size of the circuit) are guaranteed to find it. 
A takeaway from this, which may  guide future work on intrinsic saliency, is that there will not be a magical  axiomatization for a coordinate's "contribution" to the output that will also lead to efficient procedures generating succinct saliency maps. One could settle for heuristics for real-life circuits and data distributions too.
%for ReLU deep nets %\ns{existence of axiomization doesn't contradict NP-hardness of approximation?}.  
(c) Motivated by (b), we give concrete examples of circuits where saliency maps derived from existing saliency methods give no clue to what the minimal satisfying assignment is
(Section~\ref{sec:logic}). (d) Procedures for finding saliency maps using the notion of partial statistical assignment in real-life deep nets (Section~\ref{sec:procedures}). Again, these are close to masking-based methods with some subtle differences.  (e) Experiments on popular deep architectures trained on the usual datasets (CIFAR and ImageNet) illustrating properties of the partial assignments discovered by our procedure. In particular, we show that the TV regularizer (ubiquitous in computer vision) and the upsampling trick serve to make our procedure satisfy soundness condition. (f) Section~\ref{sec:linear} uses simple linear models to illustrate and explain the  above framework, including the provable role of TV regularizer for ensuring soundness even in non-vision setting.
%\ns{, suggesting that the benefit of TV might not be strictly because of the model or data distribution}. 
\fi

%\paragraph{A caution about methods and evaluations that }

\paragraph{Differences from previous work} We do not try to match the probability. Instead we maximize it, due to soundness. 

\end{comment}

==> oldintro051322.tex <==
\section{Introduction}
\label{sec:intro}
{\em Saliency methods} are a tool toward explainability, fairness,  robustness, etc. in deep learning. They are designed for two main goals: ({\bf Goal a}) {\em Understand why the deep net gave a certain answer on a particular input.} ({\bf Goal b}) {\em Convince a human overseer that the decision was correct}. The two goals can be somewhat contradictory, since the inner workings of a deep net may map poorly to human intuition. Not surprisingly, this is the source of many controversies \ns{some other term?} within the field about the very definition of saliency \ns{citation}. 

This paper restricts attention to Goal (a), and furthermore, to  the (large) class of saliency methods that 
%an input, e.g. an image, and a model, 
return an importance score for each coordinate of the input ---often visualized as a  heat map--- which captures the coordinate's importance to the final decision.\footnote{Heat maps suffice for recognition/classification tasks; other tasks may require more complex explanations.}  Early saliency methods, primarily motivated by Goal (a),  constructed such maps through an axiomatic system of ``credit attribution'' to individual input coordinates. Some involve backpropagation-like methods \citep{binder2016layer,selvaraju2016grad}, while others  use notions from cooperative game theory, such as Shapley values~\citep{lundberg2017unified,yeh2020completeness}. See \Cref{sec:prior} and \citet{samek2019explainable} for discussion of strengths and limitations of such methods. It seems generally accepted that while these methods pick up on some signal (with respect to which coordinates are most salient), they also pick up on a lot of noise \ns{citation needed}, which limits their usefulness for Goal (b).
Thus more recent methods try to find heat maps that are largely concentrated on a smaller set of pixels/coordinates.


 %tend to fall They broad definitions in machine learning. The first is visual human saliency, which attempts to predict which portions of an input, e.g. objects in a video, most capture human attention. We deal instead with the second definition, which is broadly, given 

%Some recent methods  train another deep net to produce  explanations \citep{dabkowski2017real,phang2020investigating}.
 %Often the sum of the scores equals the final decision (decision could be the output probability, or  corresponding logit).
%We refer the reader to \citet{samek2019explainable} for an extensive survey and Section~\ref{sec:prior} for a short account of such methods and controversies. % Numerous saliency methods have been proposed to learn such heat maps. 



%There are two important components in the research on saliency: {\em saliency methods} that produce such heat maps for explanations, and %{\em saliency evaluation metrics} that aim to test and compare  saliency methods.

Concurrently, an ecosystem of {\em evaluation metrics} has also sprung up to  evaluate saliency methods. These include  human evaluation \citep{adebayo2018sanity}, and comparison to certain ground truth explanations \citep{zhang2018top}. The current paper restricts attention to
{\em intrinsic} evaluations, by which we mean that evaluation uses computations involving the net itself and the heat/saliency map --- but no human evaluations or evaluations that involve training new nets. Popular intrinsic evaluations include {\em saliency metric}~\citep{dabkowski2017real} and RISE~\citep{petsiuk2018rise} \ns{Is RISE a metric or method?}.

A frequent idea in intrinsic evaluations (see \Cref{sec:stat} for references) is to create a new composite input --- or sequence of such inputs --- using the heat map and the original input, and to evaluate the original net on this composite input. For example, if $M$ is a binary vector with $1$'s in the $k$ coordinates with the highest values in the heat map, then $x \odot M$ (with $\odot$ denoting coordinate-wise multiplication) can be viewed as a masked input where only $k$ of the original coordinates of $x$ remain. (It is also popular to replace the  zeroes in this masked input with ``uninformative'' values, such as gray pixels or noisy pixels.)
This masked input is fed into the original net to check if the net outputs the same label as on the full input --- and if so one should conclude that the unmasked coordinates of $x$ were salient to the net's output. 
 This raises a potential issue of distribution shift because the net never was never trained on masked inputs. In practice, especially for image data, trained nets continue to work fine on masked inputs. (This fact is also exploited in saliency methods based upon Shapley values. \ns{citation}) Not surprisingly, recent methods for finding heatmaps use an objective that tries to directly optimize performance on such evaluations, such as ~\citep{fong2017interpretable,dabkowski2017real,phang2020investigating}, greatly outperforming older saliency methods.



%\vspace*{-0.1in}
%\subsection*{This paper}
%\vspace*{-0.1in}
 %In other words, evaluations do not involve extrinsic factors such as human judgements or retraining the net.  
 
 
 {\em Should we trust such mask-based explanations}? At first sight, this question may appear naive. In the above-described masked input
 $x \odot M$, some $k$ pixels were copied from the original image and the remaining pixels were made clearly \textquotedblleft uninformative\textquotedblright.
 Since the original net outputs essentially the same label as it did on the full image, then does this not {\em prove} that the portion that came from the mask $M$  must have {\em caused} the net's output on the full image?  The answer is \textquotedblleft No\textquotedblright, because the positions of the uninformative pixels can carry some signal.
 Many papers have noted that  optimization methods for finding subsets of salient coordinates find \textquotedblleft masks with artifacts\textquotedblright\ that look simply wrong to the human \ns{citation}.
 Indeed, we can report that in standard evaluation datasets,  it is possible to create masks out of most inputs such that the masked input  elicits high probability for a different  label from the original net prediction; see \Cref{fig:artifact-small}.  Prior works  suggested using total variation (TV) regularization while finding the masks to make them align better with human intuition, but \Cref{fig:artifact-small} shows TV regularization is not a full solution to masks that cause the net to flip the label.
 
  
 
 %{\sc move this later?} {\em 
 %the fixed {\em gaussian heatmap} that ranks pixels according to their distance to the image center turns out to be surprisingly good: it beats many  saliency methods on popular saliency evaluations on standard datasets; see \Cref{sec:expers}. } 
 
 %To be fair, the issue highlighted by \Cref{fig:artifact-small} was somewhat known, and described in ~\cite{fong2017interpretable} as \textquotedblleft masks with artifacts.\textquotedblright{}  It is recommended to use TV regularization when finding the heatmap to discourage such artifacts. However,  \Cref{fig:artifact-small} illustrates that TV regularization is not a full solution to removing artifacts: it still allows finding heatmaps that justify assigning high probability to the wrong label. 
 

\noindent{\bf Needed: Soundness.} The masked input method is trying to {\em prove} that a certain portion of the image  \textquotedblleft caused\textquotedblright\ the net's output.  Usually logical reasoning must display both {\em completeness} (i.e., all correct statements are provable) and {\em soundness} (incorrect statements cannot be proved). Checking that the net's output is essentially unchanged when switching from the full input to  the  masked input is akin to verifying {\em completeness}\footnote{Works on backprop-like saliency methods, e.g., {\sc Gradient $\odot$ Input} or {\sc lrp}, use {\em completeness} in a slightly different sense: the sum of the heat map values has to be equal to the logit value for the label. This is also motivated by the corresponding term in logic.}. But this by itself should not be convincing because, as mentioned, it is possible to use the method to find a different mask to justify another (i.e., wrong) label.   {\em Soundness}  would require verifying that the same saliency method cannot be used to produce masked inputs that make the net output a different label. 

\ns{This paragraph seems a bit misplaced here} Our view of salient pixels as \textquotedblleft proofs\textquotedblright\ of the label is termed in \citet{dabkowski2017real} as {\em Smallest Sufficient Region (SSR)} notion of saliency. They as well as~\cite{fong2017interpretable} report it to be susceptible to artifacts.  Consequently they incorporate the {\em Smallest Destroying Region (SDR)} notion:   pixels identified as most salient should be made uninformative and then one should check that the net assigns low probability for the label.   We  found soundness difficult to verify on SDR-based methods (Section~\ref{sec:expers}).
%Thus it is hard to evaluate them with respect to soundness; given labels that the net assigns low, the method is free to return the empty mask. 
The SDR notion of saliency is also implicit in many saliency evaluations,  including ROAR evaluation~\citep{hooker2019benchmark} and the Deletion Game described in Section~\ref{sec:expers}. 
%In practice, the SDR notion precludes testing for soundness, because the wrong labels have low probability to begin with, and it turns  a  big set of center pixels uninformative, thus making the probability low for all labels.  
%We note in \Cref{sec:expers} that a generic saliency map favoring central pixels---what we call the Centered Gaussian map-- is a surprisingly strong baseline in current saliency evaluations.
%Thus the SDR-based masks destroy the ability for counterfactual reasoning needed in soundness.
%A similar issue arises in 
%{\em Saliency metric}~\cite{dabkowski2017real} also ignores the mask and replaces it by the smallest rectangular box containing it. 

%i.e., labels not predicted as the most likely by the model on the full input. 
%\Cref{sec:completeness_and_soundness} formalizes soundness and proposes evaluations to test for it. 

\iffalse {\sc does following para makes sense here? else can remove it.}

Some existing evaluations like {\em ROAR}~\citep{hooker2019benchmark} indirectly address soundness  by {\em graying/noising} the pixels deemed most salient and then finding another heat map for this new input. This is repeated until no signal remains in the input ---i.e., a fresh net trained on these partially noised images cannot detect any evidence of the correct label. But note that this makes ROAR  a {\em non-intrinsic} evaluation since it involves training new nets. Furthermore, such evaluations use a subtly different notion of saliency: saliency map ends up having to include {\em all} information pertinent to the classifier's chosen label, rather than the smaller subset that was {\em sufficient} to determine the correct label.%, which means that {\em some} of the information in the grayed-out pixels was {\em essential}. 

\fi 


\begin{figure}[t!]
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{ghost_small.png}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{ghost_small_bird_frog.png}
    \end{subfigure}
    \caption{Masked CIFAR-10 images generated by our procedure with TV regularization of strength $\lambda_{TV} = 0.01$ \ns{$\lambda_{TV}$ is undefined}.
    Artifacts exist for masks generated even for incorrect labels; more examples can be found in \Cref{fig:artifact} in Appendix. The base classifier outputs the correct label on the original image (ship and bird resp.) with probability at least 0.99, and assigns probability at most $10^{-5}$ for the incorrect label (cat and frog resp.). With the generated masks, the AUC score \ns{AUC is undefined} for the correct label remains high (around 0.94 and 0.90), which corresponds to {\em completeness}, but AUC metric for the incorrect label rises tremendously (around 0.18 for cat mask, 0.71 for frog mask.) This suggests violation of {\em soundness}. }
    \label{fig:artifact-small}
    %\vspace{-0.2in}
\end{figure}

%\myparagraph{Soundness and completeness of a saliency evaluation:}
%\label{sec:soundness_completeness}

%As mentioned earlier, this paper focuses on evaluations that feed a composite input/image $x \odot M$ to the original net, where $M$ is a binary vector produced by the saliency method being evaluated.





%There could be other reasons to require some form of soundness condition in saliency evaluations. For instance, while using the classifier in the wild ---as opposed on a dataset with images of centered main objects--- multiple objects may be present in the image, and the net may not have high confidence in a single label. Then it would be reasonable for saliency methods to find evidence for all the labels present in the image. 




  
  
  

\begin{figure}[htbp] 
	\centering
	\vspace{-0.1in}
	\includegraphics[width=0.45\textwidth]{elephant-zebra.png}
	\vspace{-0.1in}
	\caption{Images containing both elephant(s) and zebra(s), and the corresponding masked ones generated by our method and the best-performing CA model in \citet{phang2020investigating}. The masks by \citet{phang2020investigating} are identical for different labels, and contains both elephant and zebra. In contrast, our method outputs decent masks for elephant and zebra accordingly. For more examples please see \Cref{fig:2label} in \Cref{sec:additionalimagenette}.  }
	\vspace{-0.1in}
	\label{fig:elezeb}
\end{figure}
  
  
%	\vspace{-0.1in}
%\myparagraph{Main contributions:}
%Motivated by the distinction between completeness and soundness, the paper makes following other contributions.
%\revise{
%In this paper we make a case for pushing saliency methods and metrics to incorporate soundness in addition to completeness.%
%We propose metrics and a method and experimentally evaluate them in comparison to previous methods and metrics, leading to some novel findings.
%Our main contributions are as follows:
%}

%	\vspace{-0.1in}
%Motivated by the above discussion, here are our contributions

%{\sc move elsewhere with a forward pointer here?}


\noindent{\bf Main Contributions of this paper:} 
\vspace{-0.1in}
\begin{itemize}[leftmargin=*]
\setlength\itemsep{0em}
\item By differentiating  {\em intrinsic} versus {\em extrinsic} evaluations (i.e., Goal (a) vs Goal (b))  the paper clarifies how to think about mask-based saliency methods. \ns{Is Goal (b) really extrinsic? It could be viewed as a goal of an intrinsic evaluation. Soundness, for instance, can also convince a human evaluator to some extent.} 
\item \Cref{sec:completeness_and_soundness} draws connections to logical proof systems and formalizes completeness and soundness in the context of saliency methods.
These are intrinsic evaluations of saliency without needing to appeal to human judgements (e.g., whether or not machine-generated masks contain artifacts).  \Cref{sec:consistency-score} introduces  {\em \cs{}}, a single number that incorporates both completeness and soundness.
% \ns{I think we do something more than this. We even clarify what an explanation or proof means in some sense.} 
%It measures the probability that the saliency map for the model prediction has the best quality compared to all other labels. 
\item \Cref{sec:procedures} revisits methods that learn masks through optimization.
Incorporating soundness, we propose a simple optimization method that maximizes the probability for any given label, rather than only the label deemed most likely by the net. \ns{citation for the other paper that does this.}
\ns{The next part about time complexity can be moved to future sections.} While this makes computation cost proportional to the number of labels,  note that this cost is only incurred while designing/evaluating the saliency method. Verification of soundness can be omitted at deployment time. (Another alternative is to verify soundness condition for top $k$ labels.)
% \item Known tricks for making masks more appealing for human evaluation (TV regularization and upsampling) are shown to have an intrinsic justification in this work: they improve soundness noticeably. \ns{Can combine this with the point below}
\item  Experiments (in \Cref{sec:expers}) estimate completeness and soundness scores for various methods. (soundness evaluation can be vacuous for some.)
Our simple method does strongly with respect to completeness and soundness as one would expect, but the slight surprise is that it performs comparably to prior masked-based methods on earlier saliency metrics as well, suggesting that soundness can be achieved without paying much in completeness.
%but also does better than those methods on the proposed consistency score. 
    %Another difference is that we use random images to fill in pixels not in the salient set when computing the objective.
    %In \Cref{tab:imagenette_main}, our method shows better soundness than previous methods, while decently matching performance existing metrics.
 \item 
 %Previous works proposed ``tricks'' like TV penalty and upscaling of masks \citep{fong2017interpretable,dabkowski2017real} that are motivated by their ability to avoid ``artifacts'' and make the saliency maps visually look better.
%    These justifications, however, are not in the spirit of an intrinsic evaluation of saliency maps.
  Heuristic choices in existing mask-based methods such as  TV regularization and upsampling, which were hitherto justified extrinsically (i.e., they make masks look natural to humans), receive  an {\em intrinsic} and precise justification: they improve soundness. %, by showing that they improve the saliency maps by making them more sound, as empirically demonstrated in 
   A theoretical result in \Cref{sec:linear} complements this experimental finding by showing that TV regularization helps saliency methods even in a simple linear classification setting, not just for vision data.
   \item Another reason for incorporating soundness in evaluations is to encourage saliency methods to react gracefully when multiple labels are correct for an image, as may happen at deployment time. 
   %Then the method should find evidence for {\em all} the labels which the net should output with reasonable confidence.We find in 
   \Cref{fig:elezeb} and \Cref{fig:2label} show images where the classifier net gave overwhelming probability to  a single label even though multiple objects were present. Our saliency method can produce different and meaningful masks for all labels that are valid.
   \ns{Extending the notion of soundness for multi-label settings is an open question.}
   %\footnote{\revise{In this paper, multiple objects in one image is not formally considered, as we assume single object classification is the prior knowledge. Therefore, either zebra or elephant in \Cref{fig:elezeb} is regarded as an incorrect label. A quick extension to the multi-object case is to define correct labels as the labels whose model probability exceeds a certain threshold. 
%Then the new definition will expect a good saliency method to provide masking explanations for elephant and zebra respectively as long as the model probability for elephant and zebra are high enough.
%Even without the extended definition of correct labels, \Cref{def:soundcompletestat} with suitable $\alpha, \beta$ already allows explanations to exist for both elephant and zebra as long as the model probability for elephant and zebra are high enough.} }, compared to prior state-of-the-art methods, that output a single mask for all labels that contains both objects (more on this in \Cref{sec:elezeb}).
\end{itemize}

	\vspace{-0.1in}
%\myparagraph{Paper outline:} \Cref{sec:prior} discusses prior works on saliency methods and evaluations. \Cref{sec:stat} delves further into the concept of completeness and soundness in the context of saliency evaluation, and describes our proposed metric of \cs{}. \Cref{sec:procedures} describes our saliency method and how it differs from prior approaches. Finally \Cref{sec:linear} describes various supportive experiments.


	\vspace{-0.1in}





%\section{Old Introduction}
% \kf{Old Intro Commented out.}

\begin{comment}
{\em Why did the deep net give a certain answer on a particular input?} {\em Saliency methods} try to provide explanations, and are thus of great interest from viewpoint of human explainability, fairness,  robustness, etc..\
 %tend to fall They broad definitions in machine learning. The first is visual human saliency, which attempts to predict which portions of an input, e.g. objects in a video, most capture human attention. We deal instead with the second definition, which is broadly, given 
This  paper restricts attention to methods that 
%an input, e.g. an image, and a model, 
return an importance score for each coordinate of the input ---usually visualized as a  heat map--- that captures its importance to the final decision.\footnote{Heatmaps suffice for usual recognition/classification tasks, but other ML tasks might require more complex explanations.} %Often the sum of the scores equals the final decision (decision could be the output probability, or  corresponding logit).
See \citet{samek2019explainable} for an extensive survey %of saliency methods and 
and Section~\ref{sec:prior} for a short account of methods and controversies. It will be good to differentiate between {\em saliency methods} ---which produce the heat map--and the {\em evaluations} of such methods. 


%We identify  two conceptually different classes of saliency methods, though their aims and methodologies (especially evaluation methodologies) of course overlap. 

%they explain the basis of an ML model's decision  by diving inside the model's computation to tease out the coordinates in the input that were most ``salient'' to the output. 

%, especially around the issue of how to evaluate saliency methods. 

The first class can be thought of as {\em intrinsic methods}: they explain the basis of an ML model's decision  by diving inside the model's computation to tease out the coordinates in the input that were most ``salient'' to the output. Doing so relies upon some {\em a priori} mathematical definition of each coordinate's ``contribution'' to the final output. Many intrinsic methods are reminiscent of backpropagation  and do "credit contribution" to each coordinate of the input roughly guided by gradient of the output with respect to the input. Some  intrinsic methods (a notable example being those relying on Shapley values from cooperative game theory) are derived from a careful axiomatization of credit attribution.
%the latter deal with the fact that the internal computation in a complicated model (say, deep net)   may not map well to human reasoning.


We refer to the second class of saliency methods as {\em human-oriented}: they avoid an {\em a priori} notion of ``contribution'' of individual coordinates of the input, and focus on 
producing human-interpretable {\em localization} of the portion  of the input germane to the output label. Recent successful methods (descended from a long tradition in computer vision) even end up  training another deep net (!) to use the classifier to compute a human-interpretable heat-map of the image regions that explain the output. Such methods do very well on a host of evaluation benchmarks, including their ability to mimic human-generated explanations. 
%There are many definitions of what should be considered important, and corresponding saliency methods have been constructed.
	
The current paper's ideas belong philosophically in the intrinsic tradition:  saliency of coordinates is defined via mathematical/logical notions that only reference the trained model. 

\iffalse
But the underlying concept of a partial assignment is very close to the masking-based concepts popular in human-oriented methods and shares their utility. We hope our formalization ---as well as supporting experiments and theory highlighting its properties--- begins to bridge the two classes of work. 
\fi

\myparagraph{Ground truth versus maximal labels versus target label.}
We evaluate both on images which the model classifies correctly, and those that it missclassifies.  Many saliency methods assume the ground truth label may not be available at test time, and we follow suit.


\myparagraph{Defining Instrinsic Saliency.}
The goal of extrinsic saliency is to highlight some relevant portion of the original input image. Given an orignal image, $X$ and a mask $M$, one can construct an image with super-imposed mask $X \odot M$ that a user may use to understand why the model made a particular decision. 
Intrinsic saliency, on the other hand, disregards use to the user, and instead has the goal of explaining a model's decision. Hence, if a model is confident on some logit $s_y$, i.e. $s_y$ is reasonably large, the saliency method should return a map certifying the value  $s_y$ (i.e. such that $f(X \odot M)$ is reasonably large). On the other hand, if $s_{y'}$ is small for some other logit, then the saliency method should not be able to find a mask $M'$ such that $f(X \odot M')$ is larger than $s_{y'}$.  If it does, then the saliency method may be explaining a belief that the model doesn't have, which would make us suspicious of its explanations in general. 

\myparagraph{Evidence of artifacts.}
Several previous works have noted the effect of mask artifacts. \citet{fong2017interpretable} noted that in an image of a maypole, the imposed mask may draw an irregular shape in the sky. \citet{dabkowski2017real} note that masks may have 'adversarial' artifacts, consisting of a few pixels that go unnoticed to humans but could destroy the model prediction. \\
Our understanding of artifacts, different from previous approaches, extends to the wrong label. Specifically, we find that un-regularized masks can be so powerful as to construct a phantom certificate for the wrong label (where $s_{y'}$ is small) such that $X \odot M'$ is large, and the resulting mask is non-trivial (consists of more than a few pixels, and can even resemble another image class.) 




Motivated by the previous observation, we consider saliency methods that learn a mask (and hence do not automatically satisfy completeness.) We introduce the notion of \emph{soundness}, that a masking method should not be able to construct a convincing explanation for the wrong label. 

We use this notion both to evaluate existing saliency methods, and to explain intrinsically various heuristic tricks that previously had only extrinsic explanations. 
%and   {\em human-oriented methods}, especially popular in computer vision, NLP etc., which try to generate human-interpretable maps and are often even evaluated with respect to ability to mimic human explanations. The two classes can and do overlap.
%Most intrinsic methods 

\myparagraph{Difficulties in working on intrinsic methods.}
A simple example can illustrate the difficulties in defining saliency  from first principles, which intrinsic methods need to. %end up having to do. 
Suppose the net's input consists of bit strings,  and it outputs $1$ iff at least $4$ input bits are $1$. What should be the saliency map for an input in which $9$ bits are $1$? Logically speaking,  highlighting any $4$ bits that are $1$ is enough to justify the answer of $1$. {\em Shapley values}, a concept from cooperative game theory, would give equal saliency to all $9$ bits that are $1$. (For simplicity we ignore here more complicated Shapley variants.) 
%A large subclass of intrinsic methods are backpropagation-like and do credit attribution roughly inspired by gradient of output with respect to input. %$\partial \text{output}/\partial \text{input}$, 
Backpropagation-like methods can give a variety of answers depending upon their details (See \Cref{sec:backpropsalmincert}), and  the final saliency map often depends upon how the net implemented its functionality (as opposed to just the input-output behavior).  The ROAR evaluation~\citet{hooker2019benchmark} would reject  maps containing fewer than six $1$'s, because it zeroes out (or greys out in case of image data) coordinates identified as most salient,  and checking if the answer on the modified input became $0$. 

%{\sc (Aside: Can we check if there are some backprop like methods that give absolutely the wrong answer, e.g. saliency to a coordinate that is $0$?)} 

%For tasks in computer vision and NLP a key objective for the saliency map is to  convince  humans that an ML model computed correctly.   This runs into the issue that a deep net's internal computation may not map well to human reasoning, and so recent successful methods \cite{} (descended from a longer tradition in computer vision) end up having to train another deep net (!) to use the first deep net to compute a human-interpretable heat-map of the image regions that explain the output. These methods do well on a host of evaluation benchmarks. 






\iffalse 

Main idea is that implicitly designers of saliency methods have been thinking of the salient portions identified in the input as a sufficient justification for the label output by the net. In other words, if $x$ is the input, and $\pi$ gives the locations and values of its most salient pixels then the pixel assignment consisting of $\pi$ in the salient pixels and grey/gaussian values in the rest is like a {\em minimal} satisfying assignment to the circuit. 
\fi 


\myparagraph{Why we focus on masking methods.}
We define masking methods similarly to \citet{phang2020investigating}; a method that attempts to learn a mask $M$ given a model $f$ and input(s) $X$. Some simple methods like LRP and Gradient $\odot$ Input for ReLU networks with no bias satisfy completeness and soundness already. However, masking methods are considered state of the art, and our focus in this work is assessing the extent to which these satisfy soundness. 

\myparagraph{Our Contributions.}
a) We introduce and motivate soundness. Since a mask-based saliency map can be viewed as a portion of the input that "certifies" the correctness of the net's output, we can view this certificate as part of a probabilistic proof system. This motivates notion of completeness (which has been discussed in previous works) and our new contribution of soundness for the saliency map. 
b) Provide a new metric (i.e., a single number) for mask-based saliency methods, which can be used to compare methods. Evaluating this metric gives new insights into efficacies of current saliency methods. 
c) We advocate for methods and evaluations for mask-based saliency  that are intrinsic ---use just the training dataset and the trained net, and does not use separately trained nets, distractor distributions, human evaluations etc. To this end, we introduce a new saliency method that does not require additional training of infillers and is fairly simple as well. 
\iffalse
We view the classifier as a circuit acting on the input.  %extends this notion to the statistical setting more relevant to machine learning. 
A central idea is a notion of saliency that involves  partial assignments that validate the label output by the circuit. This is an intrinsic notion, but  very analogous to popular {\em mask-based} explanations in the human-oriented category. (a) Sections~\ref{sec:logic} views partial assignments as precise logical concepts and defines {\em completeness} and {\em soundness} for procedures that find them. Existing saliency methods focus on at most one of these two notions, whereas both are needed.  Section~\ref{sec:stat} extends the framework to statistical learning and relates completeness and soundness to existing evaluation metrics. (b) Section~\ref{sec:logic} shows that even finding weak approximations to short partial assignments (or to deletion metrics) is computationally intractable (i.e., NP-hard) for general circuits. %of the existing saliency methods (which run in time polynomial or even linear in the size of the circuit) are guaranteed to find it. 
A takeaway from this, which may  guide future work on intrinsic saliency, is that there will not be a magical  axiomatization for a coordinate's "contribution" to the output that will also lead to efficient procedures generating succinct saliency maps. One could settle for heuristics for real-life circuits and data distributions too.
%for ReLU deep nets %\ns{existence of axiomization doesn't contradict NP-hardness of approximation?}.  
(c) Motivated by (b), we give concrete examples of circuits where saliency maps derived from existing saliency methods give no clue to what the minimal satisfying assignment is
(Section~\ref{sec:logic}). (d) Procedures for finding saliency maps using the notion of partial statistical assignment in real-life deep nets (Section~\ref{sec:procedures}). Again, these are close to masking-based methods with some subtle differences.  (e) Experiments on popular deep architectures trained on the usual datasets (CIFAR and ImageNet) illustrating properties of the partial assignments discovered by our procedure. In particular, we show that the TV regularizer (ubiquitous in computer vision) and the upsampling trick serve to make our procedure satisfy soundness condition. (f) Section~\ref{sec:linear} uses simple linear models to illustrate and explain the  above framework, including the provable role of TV regularizer for ensuring soundness even in non-vision setting.
%\ns{, suggesting that the benefit of TV might not be strictly because of the model or data distribution}. 
\fi

%\paragraph{A caution about methods and evaluations that }

\paragraph{Differences from previous work} We do not try to match the probability. Instead we maximize it, due to soundness. 

\end{comment}

==> table_fig/imagenet_rn50_table.tex <==
\begin{table}[t!]
\begin{center}
	\caption{Performance of our method on ImageNet and ResNet-50 model and some baselines on various intrinsic saliency metrics proposed in prior work.  We find that while both our masks (learned with and without TV) have very good performance on the insertion metric, the mask learned with TV has much better performance on the saliency metric. The deletion metric is uninformative in most cases, since most methods are as good (or worse) compared to a random mask.}
	\label{table:metrics}
	\vspace{0.1in}
\begin{tabular}{ |c|c|c|c| c| c| } 
 \hline
 & Gradient $\odot$ Input & Our method & Our Method & Real Time & Random \\ 
 &  & ($\lambda_{TV}=0.01$) & ($\lambda_{TV}=0$) & saliency &   \\ 
 \hline
 Deletion $\downarrow$      &     0.1451      &  0.1832   &     0.2067     &    0.1851     &  0.1843   \\

Insertion (blur) $\uparrow$      &  0.5434      &  0.8363   &   0.8673  & 0.6857 &0.3562 \\ 
Insertion (gray) $\uparrow$      &  0.3716  & 0.7401   &    0.8857        & 0.4873 & 0.1835 \\ 
Saliency Metric $\downarrow$    &   0.2549  &  0.2019    & 0.2604          &     0.2943  &  0.2584 \\ 
 \hline
\end{tabular}
\label{table:ImageNetResNet-50}
\end{center}
\end{table}

==> table_fig/imagenette_c_complete_sound.tex <==

\begin{table*}[htbp]
    \centering
    \caption{Completeness, soundness and \cs{} for each saliency method on Imagenette-Corner, averaged over test samples. We compute completeness on labels that the model predicts, and the minimum soundness among the incorrect labels (w.r.t. the model prediction).  The best two of each column are marked bold. Consistency scores are highly correlated to completeness/soundness in the table. $s=4$ indicates upsampling as in Section \ref{sec:procedures}. The numbers for Centered Gaussian drop compared to Imagenette.}
    \label{tab:imagenette_c_complete_sound}
    \begin{tabular}{|c|c |c |c|}
    \hline
         & Completeness of  & Worst soundness of & Consistency \\
         & model prediction & the incorrect labels & Score \\
    \hline
    Gradient $\odot$ Input & 0.41 &  0.80 & 81.0\% \\
    \citet{dabkowski2017real} & 0.44  & 0.79 & 82.9\% \\
    \citet{fong2017interpretable} & 0.47  & 0.51 & 80.1\% \\
    \citet{phang2020investigating} & \bf 0.63  & \bf 0.84 & \bf 85.4\% \\
    \hline
    Ours ($s=4$) & {\bf 0.67} & \bf 0.89 & \bf 85.6\% \\
    \hline
    Random & 0.26 & 0.65 & 76.5\% \\
    \revise{Centered Gaussian} & 0.43 & 0.58 & 79.7\% \\
    \hline
    \end{tabular}
    %\resizebox{\textwidth}{!}{
    % \begin{tabular}{|c|c c c|c|}
    % \hline
    %      & Completeness of  & Average soundness of  & Worst soundness of & Consistency \\
    %      & model prediction & the incorrect labels & the incorrect labels & Score \\
    % \hline
    % Gradient $\odot$ Input & 0.41 & \bf 0.98 & 0.80 & 81\% \\
    % \citet{dabkowski2017real} & 0.44 &  0.97 & 0.79 & 82.9\% \\
    % \citet{fong2017interpretable} & 0.47 & 0.93 & 0.51 & 80.1\% \\
    % \citet{phang2020investigating} & \bf 0.63 & {\bf 0.98} & \bf 0.84 & \bf 85.4\% \\
    % \hline
    % Ours ($s=4$) & {\bf 0.67} & {\bf 0.99} & \bf 0.89 & \bf 85.6\% \\
    % \hline
    % Random & 0.26 & 0.95 & 0.65 & 76.5\% \\
    % \revise{Centered Gaussian} & 0.43 & 0.95 & 0.58 & 79.7\% \\
    % \hline
    % \end{tabular}
    %}
\end{table*}

==> table_fig/imagenette_complete_sound_1_table.tex <==
\begin{table*}[ht]
    \centering
    \caption{Completeness, soundness and best effort, $\epsilon_1=0.01$}
    \label{tab:imagenette_complete_sound}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c | c|c|}
    \hline
         & Completeness of & Worst Completeness of   & Worst Completeness of & Worst Soundness of \\
         & model prediction & all labels              &  the incorrect labels & all labels \\
    \hline
    Gradient $\odot$ Input & 0.56  & 0.56 & 0.9982 & 0.80 \\
    \citet{dabkowski2017real} & 0.58  & 0.58 & 0.9983 & 0.82 \\
    \citet{fong2017interpretable} & 0.57  & 0.57 & 0.9984 & 0.60 \\
    \citet{phang2020investigating} & 0.71  & 0.71 & 0.9983 & 0.84 \\
    \hline
    Ours ($s=1$) & 0.86 & 0.86 & 0.9993 & 0.58 \\
    Ours ($s=4$) & 0.84 & 0.84 & 0.9989 & 0.84 \\
    Ours ($s=4$, gray) & 0.64 & 0.64 & 0.9983 & 0.76 \\
    Ours ($s=4$, $\lambda_{TV}=0.001$) & 0.87 & 0.87 & 0.9993 & 0.65 \\
    \hline
    Random & 0.38 & 0.38 & 0.9976 & 0.69 \\
    \revise{Centered Gaussian} & 0.64 & 0.64 & 0.9979 & 0.71 \\
    \hline
    \end{tabular}
    }
\end{table*}

==> table_fig/imagenette_complete_sound_table.tex <==
\begin{table*}[ht]
    \centering
    \caption{Completeness, soundness and \cs{} for each saliency method on Imagenette, averaged over test samples. Completeness is computed on labels that the model predicts. For soundness, we compute the minimum one among all incorrect labels (w.r.t. the model prediction). Soundness scores of past methods except Gradient $\odot$ Input should be {\bf treated as meaningless} as explained in Section~\ref{subsec:comp}. The best two of each column are marked bold. Consistency scores are highly correlated to completeness/soundness in the table. $s=4$ indicates upsampling as in Section \ref{sec:procedures}.}
    \label{tab:imagenette_complete_sound}
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c | c|c|}
    \hline
         & Completeness of   & Worst soundness of & Consistency \\
         & model prediction &  the incorrect labels & Score \\
    \hline
    Gradient $\odot$ Input & 0.54  & 0.83 & 84.1\% \\
    \citet{dabkowski2017real} & 0.56  & 0.85 & 85.7\% \\
    \citet{fong2017interpretable} & 0.53  & 0.61 & 84.5\% \\
    \citet{phang2020investigating} & 0.71  & \bf 0.87 & \bf 87.1\% \\
    \hline
    Ours ($s=1$) & {\bf 0.85} & 0.61 & 86.2\% \\
    Ours ($s=4$) & {\bf 0.83} & \bf 0.89 & \bf 88.0\% \\
    Ours ($s=4$, gray) & 0.64 & 0.79 & 86.7\% \\
    Ours ($s=4$, $\lambda_{TV}=0.001$) & 0.87 & 0.71 & 87.2\% \\
    \hline
    Random & 0.35 & 0.70 & 82.9\% \\
    \revise{Centered Gaussian} & 0.63 & 0.74 & 86.7\% \\
    \hline
    \end{tabular}
    %}
\end{table*}

==> table_fig/tvfig.tex <==
%
\begin{figure}[!t]
	\centering
	\includegraphics[scale = 0.8]{fig1_nosparse.png}
	\includegraphics[scale = 0.8]{fig2_nosparse.png} 

		\caption{ \textbf{Top-3 rows}: Masks validating the correct label of ImageNet images using \Cref{sec:procedures}. Pixels outside the ``salient set'' $S$, as determined by the mask, are rendered as grey. Size of $S$ (as \% of total pixels) appears below the images. Value of TV regularizer shown above each column corresponding to (0,.001,.01,.1). Original image rendered in last column. True labels with original model probabilities are shown in the rightmost column. AUC Insertion score when the mask is found by the procedure in Section \ref{sec:procedures} shown on y-axis of each image, \textbf{Bottom-3 rows}: Masks validating the second-best label, which appears on the right along with original model probability of that label. Insertion metric when the mask is found by fitting the second best label under the procedure in Section \ref{sec:procedures} is shown on the y label of each plot. We find that increasing the TV regularizer makes the resulting assignment more sound.}
		\label{fig:tvfig}
    % \vspace{-0.2in}
\end{figure}
